Investigating Crowdsourcing Protocols for Evaluating the Factual Consistency of Summaries

Current pre-trained models applied to summarization are prone to factual inconsistencies which either misrepresent the source text or introduce extraneous information. Thus, comparing the factual consistency of summaries is necessary as we develop improved models. However, the optimal human evaluation setup for factual consistency has not been standardized. To address this issue, we crowdsourced evaluations for factual consistency using the rating-based Likert scale and ranking-based Best-Worst Scaling protocols, on 100 articles from each of the CNN-Daily Mail and XSum datasets over four state-of-the-art models, to determine the most reliable evaluation framework. We find that ranking-based protocols offer a more reliable measure of summary quality across datasets, while the reliability of Likert ratings depends on the target dataset and the evaluation design. Our crowdsourcing templates and summary evaluations will be publicly available to facilitate future research on factual consistency in summarization.

==> summ - emnlp2021/old-related-work.tex <==
% \section{Related Work}
% Crowdsourcing judgments provide convergent evidence and can help overcome the limitations of automated metrics \cite{belz-kow-2011-discrete}, but there is little agreement on how to perform a crowdsourcing evaluation \cite{amidei-etal-2018-rethinking}. \citeauthor{shrout1979intraclass,landis1977measurement} use intra-class correlation (ICC) to measure the reliability across multiple raters. \citeauthor{steen2021evaluate} reported split-half reliability (SHR) in addition to Krippendorff's alpha \cite{krippendorff2018content}. They also added the dimension of annotator workload as a primary determinant of cost to the comparison. This work showed that ranking-style evaluations are more reliable and cost-efficient for coherence, similar to \cite{novikova-etal-2018-rankme, sakaguchi-van-durme-2018-efficient} but worse than Likert in the repetition quality dimension. This work is most similar to ours, but their experiments included neither factual consistency nor Best-Worst ranking. Within dialogue systems, 
% \citeauthor{Santhanam2019TowardsBE} conducted experiments in which the Likert scale and BWS achieve very close consistent ratings, with BWS achieving higher inter-rater agreement. We build on these related works to examine Likert scaling and BWS for factual consistency in summarization.

==> summ - emnlp2021/save.tex <==
% \newcommand{\Interchangerate}{
% \begin{table}[t!]
% \centering
% \resizebox{\columnwidth}{!}{\begin{tabular}{c | c c c |  c c c} \Xhline{3\arrayrulewidth}
%             &  \multicolumn{3}{c|}{CNN/DM} &  \multicolumn{3}{c}{XSum}  \\ 
%             \multirow{0.3cm}{*}{ }  & BWS & Likert-5 & Likert-10 & BWS & Likert-5 & Likert-10 \\ \hline
%   \multirow{0.3cm}{*}{}Change Rate     & 74.71\%   & 87.75\% &    96.00\%  &   70.25\% & 92.25\%   &  96.25\% \\
%   &  -  & 29.76\%  &   25.44\%   &  - & 34.98\%  &  33.79\% \\
%  \Xhline{2\arrayrulewidth}
% \end{tabular}}
% \caption{Inter-annotator average change rate and range across BWS, Likert-5 and Likert-10 evaluations. For Likert, \texttt{Average Change Rate}: what percentage of the total summaries have different scores given by different annotators,
% \texttt{Average Change Range}: what percentage of the score is changed in each change. For BWS, \texttt{Average Change Rate}: what percentage of the total summaries have different rankings given by different annotators.}
% \label{tab:model_scores}
% \end{table}
% }
% \section{Experiments}
% \RougeScores
% Each study contains 100 original passages, and 400 summaries generated from four pre-trained models. We randomly sample 100 documents from the corpus with corresponding summaries from models to form the item set for all our studies.
% To describe the design of our studies sufficiently, we demand 3 judgments per summary to mirror a common setup in manual evaluation, while each annotator only can annotate 5 summaries, neither 3 annotators who did all judgments in one extreme nor a study with 300 distinct annotators. And we ensure a sufficient total number of annotators by using a block design. We separated our corpus into 20 blocks of 5 documents and included all 4 generated summaries for each document in the same block, which results in 5 × 4 = 20 summaries per block.



% \textbf{Likert Scale (LS)} is typically used in experiments for crowdsourcing human evaluation \cite{DBLP:conf/ecir/AsgharPHJM18}. 
% Best-worst scaling (BWS) is a specific type of ranking-oriented evaluation that requires annotators to specify only the first and last rank \cite{hollis2018best, kiritchenko-mohammad-2017-best}. 

% \textbf{Corpus and Systems.}  
% Models: 
% % 
% We conduct our experiments on the following
% models' output: \textbf{BART}~\cite{lewis-etal-2020-bart}, a denoising autoencoder for pretraining sequence to sequence tasks which is applicable to both natural language understanding and generation tasks; \textbf{ProphetNet}~\cite{qi-etal-2020-prophetnet}, which is a pre-trained encoder-decoder model and can predict n-future tokens for “ngram” language modeling instead of just the next token;
% \textbf{PEGASUS}\cite{pmlr-v119-zhang20ae}, a model pretrained with a novel objective function designed for summarization by which important sentences are removed from an input document and then generated from the remaining sentences; and 
% \textbf{BERTSUM}~\cite{liu-lapata-2019-text}, a two-stage fine-tuning approach
% where the BERT-based encoder is first fine-tuned
% on the extractive summarization task and then on
% the abstractive sumarization task with the decoder.



% XSum~\cite{narayan-etal-2018-dont} consists of 227K online articles from the British Broadcasting Corporation (BBC), which contains professionally written single-sentence summaries. After the preprocessing, there are 226,677 article, summary data pairs, where the source input is the news article, and the target output is a single-sentence summary.
% % 
% Krippendorff's alpha ($\alpha$) is a reliability coefficient developed to measure the agreement among multi observers~\cite{krippendorff2011computing}.
% % 

% \LikertDistributions
% \ModelScores



% % \begin{table}[htbp]
% % \centering

% % \begin{tabular}{c|ccc|cc}\toprule\hline 



% %  &\multicolumn{3}{c|}{XSum} & \multicolumn{2}{c}{CNN/DN} \\

% % \multirow{0.3cm}{*}{Models}       & BWS& Likert & Likert-10 & BWS& Likert  \\\hline 
% % PEGASUS       &  3.247^{\color{cyan}3}   &    3.350^{\color{red}1} &6.247^{\color{cyan}2}  &  3.230^{\color{cyan}2}   &    3.887^{\color{cyan}2}   \\
% % ProphetNet    & 3.360^{\color{cyan}2}    &    3.293^{\color{cyan}3} &6.427^{\color{cyan}2}  & 3.100^{\color{cyan}3}    &    3.860^{\color{blue}4}    \\
% % BART          &  3.570^{\color{red}1}   &    3.433^{\color{cyan}2} & 6.937^{\color{red}1} &  3.593^{\color{red}1}   &    4.017^{\color{red}1}  \\
% % BERTSUM &  2.827^{\color{blue}4}    &    2.790^{\color{blue}4}  & 5.163^{\color{blue}4} &  3.087^{\color{blue}4}    &    3.863^{\color{cyan}3}   \\  \hline \hline \toprule
% % \end{tabular}

% % \caption{The average Likert scores and the
% % average rank for all systems on XSum and CNN/DM.}
% % \end{table}




% \begin{table}[htbp]
% \centering
% \begin{tabular}{c|c|c}\hline \hline
% krippendorff        & XSum & CNN/DM \\\hline 
% BWS     &    0.2477 & \textbf{0.1582}\\ 
% Likert-5 &  0.2202  & 0.0443  \\

% Likert-10 &  \textbf{0.2951}  & -   \\
% \hline \hline
% \end{tabular}
% \caption{Instance-level reliability computed by Krippendorff 's alpha ($\alpha$) on the CNN/DM and XSum.}
% \end{table}



% \begin{table}[htbp]
% \centering
% \begin{tabular}{c|c|c}\hline\hline
% SHR & XSum         &  CNN/DM\\\hline 
% BWS      & 0.90314 &    \textbf{0.87657} \\ 
% Likert & \textbf{0.92777}  &  0.45619  \\
% Likert-10 &  \textbf{0.94853}  & -  \\

% \hline\hline
% \end{tabular}
% \caption{System-level split-half reliability computed by Split-Half Reliability (SHR) on the CNN/DM and XSum.}
% \end{table}

